Guessing Winning Policies in LTL Synthesis by Semantic Learning

We provide a learning-based technique for guessing a winning strategy in a parity game originating from an LTL synthesis problem. A cheaply obtained guess can be useful in several applications. Not only can the guessed strategy be applied as best-effort in cases where the game's huge size prohibits rigorous approaches, but it can also increase the scalability of rigorous LTL synthesis in several ways. Firstly, checking whether a guessed strategy is winning is easier than constructing one. Secondly, even if the guess is wrong in some places, it can be fixed by strategy iteration faster than constructing one from scratch. Thirdly, the guess can be used in on-the-fly approaches to prioritize exploration in the most fruitful directions. In contrast to previous works, we (i)~reflect the highly structured logical information in game's states, the so-called semantic labelling, coming from the recent LTL-to-automata translations, and (ii)~learn to reflect it properly by learning from previously solved games, bringing the solving process closer to human-like reasoning.

==> 0_macros.tex <==
% == LATEX
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%\newcolumntype{L}{X}
%\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
%\newcolumntype{C}{>{\centering\arraybackslash}X}

\RequirePackage{amsmath}
\RequirePackage{amssymb}

% == SYMBOLS

\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}

% == BASIC OPERATORS

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\pospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\negpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\inner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\cardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\tuple}{(}{)}
\DeclarePairedDelimiter{\listt}{[}{]}


% == SETS OPERATORS

\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}


% == BASIC SETS

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}


% == OPERATORS

\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum

% == LOGIC

% lor, land, lnot etc already defined
\newcommand{\lOr}{\bigvee}
\newcommand{\lAnd}{\bigwedge}
\newcommand{\lfalse}{\texttt{ff}}
\newcommand{\ltrue}{\texttt{tt}}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\newcommand{\LTL}{\operatorname{LTL}}
\newcommand{\CTL}{\operatorname{CTL}}
\newcommand{\PCTL}{\operatorname{pCTL}}

\newcommand{\ltlNext}{\operatorname{\mathbf{X}}}
\newcommand{\ltlFinally}{\operatorname{\mathbf{F}}}
\newcommand{\ltlGlobally}{\operatorname{\mathbf{G}}}
\newcommand{\ltlUntil}{\mathbin{\mathbf{U}}}
\newcommand{\ltlWuntil}{\mathbin{\mathbf{W}}}
\newcommand{\ltlRelease}{\mathbin{\mathbf{R}}}
\newcommand{\ltlSrelease}{\mathbin{\mathbf{M}}}
\newcommand{\ltlLanguage}[1]{\mathcal{L}(#1)}
\newcommand{\true}{\texttt{tt}}
\newcommand{\false}{\texttt{ff}}
\newcommand{\trueness}{t}

\newcommand{\Alphabet}{\Sigma}
\newcommand{\AP}{\mathsf{AP}}

\DeclareMathOperator{\subformulas}{sub}
\DeclareMathOperator{\topformulas}{top}

\DeclareMathOperator{\satisfying}{sat}

% == COMPLEXITY

\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\mathbf{coNP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}

% == GAMES

\newcommand{\G}{\mathcal{G}}
\newcommand{\Vertices}{V}
\newcommand{\Edges}{E}
\newcommand{\VertexPlayer}{P}
\newcommand{\EdgesSys}{E_\sys}
\newcommand{\EdgesEnv}{E_\env}
\newcommand{\initialvertex}{v_0}
\newcommand{\play}{\rho}
\newcommand{\Plays}{\mathfrak{P}}
\newcommand{\player}{p}
\newcommand{\strategy}{\sigma}
\newcommand{\priorities}{\mathfrak{p}}

\newcommand{\sys}{\mathcal{S}}
\newcommand{\env}{\mathcal{E}}
\newcommand{\VerticesSys}{\Vertices_\sys}
\newcommand{\VerticesEnv}{\Vertices_\env}

\newcommand{\GExt}{\mathsf{Ext}}
% == OTHER

\DeclareMathOperator{\obligationSetFormula}{\emph{osf}}
\DeclareMathOperator{\someAssignment}{\mathcal{A}}



\newcommand{\para}[1]{{\smallskip\noindent\textbf{#1}}}



==> 3_ideas.tex <==
\section{Our Contributions}

Section content
\begin{itemize}
	\item Overall goal: predict initial strategies for SI to speed up solving, or more general, learn what winning decisions in labelled parity games look like.
	
	\item breaking the overall problem down to a local preference problem (which we can break even further down into pair preferences)
	
	\item Chain of prerequisites:
	\item For that matter, we want to pairwise rank the edges of system states to find the best choice for each state.
	\item for that we need a pair classifier
	\item as there are more things to consider than just trueness, we need more features.
	\item as it is unclear how to evaluate all features at the same time, we need ML
	\item for ml we need GT
\end{itemize}

\subsection{Ground truth}
\begin{itemize}
	\item you might think this is trivial: just use SI and winning is good, loosing is bad
	\item problem: $a \oplus \ltlNext b$
	\item so set every edge that somehow wins to good?
	\item also not good (e.g. $a\lor \ltlGlobally\ltlFinally b$ going for the immediate win with a is best but if you don't play a, playing b is still better than not playing b)
	\item we want $f:\Edges \to \Reals$ (or for simplicity $[0,1]$) where $f(e_1) < f(e_2)$ means $e_2$ is better than $e_1$.
	I.e.\ a ranking among all edges of a system state.
	\item our approach to GT:
	\begin{itemize}
		\item Gametree unfolding with min-max gamevalue propagation and beta decay to prioritize edges leading to small solutions.
		\item if loop is closed, great! Assign the node that closed it 0 or 1 depending on whether it was winning.
		However, already for medium sized games this is completely infeasible to do exhaustively.
		\item Thus we compute a monte carlo simulation based GT which we incorporate in two ways:
		\begin{itemize}
			\item after some maximal depth is reached in the gametree unfolding, simply use the MC GT value as an approximation.
			\item decrease the branching factor of the tree by only giving the environment access to the edge with the lowest MCGT or the two edges with the lowest MC GTs if the decision is close ($\Delta < 0.02$)
			\item i know the latter sounds stupid but allows for a much higher depth and apparently works quite well in practice (G7 was much better than G3 in thesis, otherwise G7 could not exist)
			\item small problem with the former: we use monte carlo simulation without the starting path of the game tree due to practical reasons; this occasionally leads to problems (final section thesis)
		\end{itemize}
		
		\item smart MC works as follows:

		\begin{itemize}
			\item starts in some state where the first edge choice is fixed.
			\item after the first edge, plays randomly though the game with the following restrictions for each player:
			\item env:
			\begin{itemize}
				\item plays optimal, i.e.\ wins every state it can win. (return 0 immediately if a lost state is reached)
				\item tries to delay losing as long as possible in states the system wins for beta decay to function properly.
			\end{itemize}
			\item sys:
			\begin{itemize}
				\item always finds one-step-trivial-wins
				\item never plays one-step-trivial-losses
				\item randomly plays among the non-insta-losing edges
			\end{itemize}
			\item if a loop is closed, we can decide whether the play is winning or losing
			\item ultimately, we divide the number of winning simulated plays by the total number of plays which yields 
			\item smartMC also uses beta decay, i.e. a losing play is still value 0 but a winning play is $\beta^{\text{length}}$
			
			\item SCC optimization:
			(not sure if this is implementation or even implementation detail.
			I think it is at least an interesting side fact)
			\begin{itemize}
				\item we compute the scc decomposition of the game and a topological ordering among them
				\item we make sure to compute the MCGT in for all edges in that topological order, i.e.\ first compute the MCGT in the BSCCs.
				\item whenever a simulation leaves the SCC of the edge it originated from, due to the topological ordering, we reach a state of an SCC that has already been done.
				Then we reuse the GT value there as result of that path, which implicitly yields us a lot of simulations for the original edge.
				Returning this as path result also works perfectly with the betas of the decay.
			\end{itemize}
		\end{itemize}
	\end{itemize}
\end{itemize}

{\color{red} 
This requires the following prelims
\begin{itemize}
	\item Parity Game and LTL
	\item semantic labelling for instawinning/losing
	\item tree unfolding (extensive form games) and min-max-Algorithm (might be known enough to just reference it here?)
	\item beta decay (can probably be explained here as well)
	\item monte carlo simulation (?)/ Strategies, for best effort strategy of environment
	\item If Scc optimization shall be part of this section: SCCs, topological order(?)
\end{itemize}
}

\subsection{Features}
General Disclaimer: No feature tries to be a good heuristic on its own.
There will always be formulae where the feature is misleading.
Only the combination of all features will yield the desired outcome.
\begin{itemize}
	\item base features that can be applied to any formula:
	\item for all of them we can compute the feature value of the successor of an edge or the change in that value along an edge
	\item if we apply them to monitors, we have to aggregate them as we only want one feature value per state (we always do weighted average to emphasize the monitors higher in the list)
	\item if we apply it to the \enquote{next} part of all the monitors, we have to aggregate twice.
	We use average over the next list, and once again waverage over the monitors
	\begin{itemize}
		\item syntactic:
		\begin{itemize}
			\item conjuncts: 
			\begin{itemize}
				\item How: number of conjuncts if top level operator is $\land$ else 1
				\item Intuition: low number of conjuncts is less constrained. Reducing conjuncts along an edge might correspond to achieving subgoals
				\item Note that this is highly dependent on the way how the semantic labelling works (i.e. masterformula is to be satisfied/ is  a list of subtasks, especially in practical formulas)
				\item Stress: formulae within the automaton are syntactical derivations from the input formulae, the human bias in these formulae is present in the entire automaton
			\end{itemize}
			\item disjuncts: 
			\begin{itemize}
				\item How: number of disjuncts if top level operator is $\lor$ else 1
				\item Intuition: More disjuncts means more options.
			\end{itemize}
			\item goals: 
			\begin{itemize}
				\item How: sounds stupid and also never documented in any report, yet it was selected by feature elimination:
				\begin{enumerate}
					\item find a minimal number of non-(cosafety/safety) subformulae that need to be fulfilled for the overall formula to be satisfied
					\item return the number of (safety/co-safety) formulae that need to be fulfilled in addition th that as feature value (and omit the original minimum completely for some reason?)
				\end{enumerate}
				\item Intuition: None, it's stupid to use the number of safety/cosafety instead of the number of non safety subgoals (the thing you minimized)
				
			\end{itemize}
			\item height: 
			\begin{itemize}
				\item How: height of syntax tree
				\item Intuition: smaller formulae are simpler 
			\end{itemize}
			\item tempOps:
			\begin{itemize}
				\item How: count temporal operators
				\item Intuition: same as height but also in the width of the syntax tree
			\end{itemize}
			\item systemControlProp (literally variable counting)
			\begin{itemize}
				\item How: divide number of system variables by number of total variables
				\item Intuition: more system variables means more influence on the formula
			\end{itemize}
		\end{itemize}
		\item semantic
		\begin{itemize}
			\item trueness
			\begin{itemize}
				\item How: ATVA
				\item Intuition: how easy is it to satisfy the formula
			\end{itemize}
			\item envControl/syscontrol binary
			\begin{itemize}
				\item How: Inductive function as described in Backs report (Appendix I guess).
				1 if the sys/env can force the formula to true/false
				\item Intuition: approximation whether the system can force the formula to true r the environment can force it to false.
				Play towards states where systemcontrol is 1. Avoid states where envControl is 1.
			\end{itemize}
			\item sysControl continuous
			\begin{itemize}
				\item How: more complex inductive function as described in thesis (Appendix I guess).
				Approximate Binary Temporal operators by 0.0/0.5/1.0 depending on binary env/sys control.
				propagate values through unary operators.
				For disjunction/conjunction: monotonous functions (can be written nicely by assuming the $\phi_i$ are ordered by their values)
		
				\item Intuition: more information than the binary control features by introducing much more intermediate levels.
			\end{itemize}
			\item obSet + \{trueness,sysControlContinuous, sysControlProp\}
			\begin{itemize}
				\item Obligation set: an assignment that can be played indefinitely and satisfies the formula
				\item ObSetFormula: a formula that is satisfied by exactly all assignments that are obligation sets.
				\item efficiently computable by substitution 
				\item this new formula can again be bombarded by features that are applicable to formulae
				\item we chose:
				\begin{enumerate}
					\item trueness (Intuition: the easier the formula is to satisfy, the more obligation sets there are, the more likely it is to be able to force one)
					\item syscontrol (continuous and prop) (Intuition: the better the system can control the ObSetFormula, the likelier it is to be able to enforce one)
				\end{enumerate}
			\end{itemize}
		\end{itemize}
	\end{itemize}
	\item edge specific features 
	\begin{itemize}
		\item priority
		\item progress features: All of those are monitor depended, so aggregation is needed.
		\begin{itemize}
			\item makesProgress: telling if any of the currently monitored co-safety formulas made any progress along the edge. (Intuition: Sometimes the SVM procrastinates and avoids aiming for a complicated formula somewhere in the successor at the cost of not making any progress. To avoid only focusing on the formula, this feature is added to teach the SVM that progress is important.)
			\item coSaSucc + \{noPunish, smallPunish\}: This is the percentage of succeeded co-safety formulas. In case a monitor fails it gets a value of -1 to distinguish it from monitors without progress (Failing is not always reflected in the priority, if a higher monitor succeeds or also fails, but should be avoided). However, some monitors reappear at the end of the list (If there is an F somewhere). This monitors can be handled without punishment (apart from possibly the priority) or small punishments, usually -0.5.
		\end{itemize}
		\item oneStepRec
		\begin{itemize}
			\item idea/intuition: try to give a recommendation of what to play in the next step by passing messages through the syntax tree.
			Then assign feature values to the edges depending on how well they fit this recommended assignment.
			\item exact functionality should probably be in appendix
			\item note that the assignment itself often does not make too much sense. However, how well an edge matches this kind of recommendation gives information to the model to deal with.
			\item here Future work could be interesting by having different kinds of these recommendations that focus on different things and the combination of all of them yields information
		\end{itemize}
	\end{itemize}
\end{itemize}

{\color{red}
This requires the following preliminaries
\begin{itemize}
	\item Intuition on how the semantic information looks like.
\end{itemize}
}

\subsection{Model: the PairClassifier SVM}
Probably rather short section
\begin{itemize}
	\item takes pairs of edges as input (concat their features)
	\item choses best edge/ranks edges by looking at all combinations of edges and summing up the confidences for or against them
\end{itemize}

{\color{red}
	This requires the following preliminaries
	\begin{itemize}
		\item :)
	\end{itemize}
}


In this section, we explain the central ideas of our contributions.
First, we highlight the peculiarities of the mentioned labelling function.
Then, we introduce the concept of \emph{trueness}, which we directly use to augment strategy improvement.
Finally, we explain our adaptation of Q-learning to parity games and how we derive a semantic reward signal from the labelling, using trueness.

\subsection{Input Details} \label{sec:contributions:input}

We assume that we are given a parity game, where each vertex is labelled by a structured list of LTL formulae.
The labelling corresponds to the remaining goals to be achieved by the system player (or violated by the environment player).
More precisely, the labelling consists of one \emph{master formula} and potentially several \emph{monitors}.
The master formula tracks the \enquote{overall progress} and all finitely achievable parts of the formula.
In particular, the master formula \true{} corresponds to the formula being satisfied by the prefix, analogously \false{} corresponds to a falsified formula.
The system player automatically wins if a vertex labelled with \true{} is reached and, similarly, loses on a \false{} vertex.
In the special case of reachability or safety specifications, the labelling actually only consists of the master formula.

For more complex specifications, the labelling also exhibits a more intricate structure.
Intuitively, there is one monitor for each sub-formula which needs to be satisfied infinitely often (liveness conditions) or may only be violated finitely often (safety conditions).
Each monitor tracks a list of formulae which have to be fulfilled in order to satisfy its overall goal.
The monitors are ordered according to an appearance-record style construction.
\enquote{Failing} monitors emit a bad priority and are moved at the beginning of the list, succeeding monitors instead emit a good priority.
Both priorities are based on the respective monitor's position in the list.
Intuitively, for a fixed word $\omega$, all monitors which only fail finitely often eventually are ranked higher than all the monitors which fail infinitely often.
Thus, if such a non-failing monitor emits a good priority, it overrules all of the failing monitors' bad priorities.

Consider, for example, the formula $\ltlFinally \ltlGlobally a$, meaning \enquote{eventually, $a$ appears every step}.
Here, there is no ultimate \true{} or \false{} vertex, since this formula cannot be satisfied or violated by any finite prefix.
The construction gives us $\ltlFinally \ltlGlobally a$ as master formula and $\ltlGlobally a$ as a monitored goal.
Whenever we see a $\lnot a$, this monitor would fail, emit a bad priority, and move to the front of the list.
Dually, for every $a$, it emits a good priority.

The details of this construction are described in \cite{DBLP:conf/tacas/EsparzaKRS17}.
It is implemented in the tool \texttt{Rabinizer} \cite{DBLP:conf/cav/KretinskyMSZ18} %\texttt{Rabinizer} \cite{DBLP:conf/atva/KretinskyMS18}, which we use as base library 
which we use for our constructions.
An online demo thereof is located at \url{https://owl.model.in.tum.de/try/}. %TODO FINAL: rabinizer. ...
A simplified example can be found in \cref{fig:example_labelling} later on.

\subsection{(Co-)Safety games}

Recall that for these games, the labelling we obtain is a single LTL formula per vertex.
The system player wants to reach the $\true$ vertex and avoid the $\false$ vertex.
Consequently, the system player naturally is interested in taking \enquote{trueness-maximizing} edges, analogously the environment player wants to move away from $\true$.
This simple observation directly leads us to the concept of \emph{trueness}.

\subsubsection{Trueness} of an LTL formula $\trueness : \LTL \to [0, 1]$ intuitively denotes how \enquote{close} a given formula is to being satisfied.
We compute this value by treating the formula as purely propositional, i.e. each temporal operator is considered to be a fresh variable.
Formally, given an LTL formula $\phi$, we interpret it as a propositional formula over $\Alphabet = 2^{\AP \union \topformulas(\phi)}$.
For this formula, we then determine and scale the ratio of satisfying assignments, i.e.\ $\trueness(\phi) := \cardinality{\satisfying(\phi)} / \cardinality{\Alphabet}$.
This value can be computed efficiently by representing the formula as \emph{binary decision diagram (BDD)}\cite{DBLP:reference/mc/Bryant18}, as implemented in \texttt{Rabinizer}.
Even for formulae with several hundred syntax elements the trueness is computed virtually instantaneously.

At first, this notion may seem rather unintuitive, since the temporal aspect of a formula is not necessarily reflected by the trueness value.
For example, the formula $\phi = \ltlGlobally a \land \ltlGlobally \lnot a$ has a trueness value of $\trueness(\phi) = \frac{1}{4}$, but actually is unsatisfiable.
Nevertheless, trueness proves to be a surprisingly good initialization heuristic, which we explain in the following and further demonstrate in our evaluation.

One particular reason for its performance in our application is due to the way the labelling is constructed.
In particular, temporal operators are \enquote{unfolded} as an essential step of the construction.
For example, the formula $\ltlGlobally a$ is unfolded to $a \land \ltlGlobally a$ while $\ltlFinally a$ yields $a \lor \ltlFinally a$ and $a \ltlUntil b$ gives $b \lor (a \land (a \ltlUntil b))$.
The unfolded variants are semantically equivalent to the original formula, but provide us with a one-step propositional \enquote{approximation} of the temporal operators.
The above $\phi$ then is unfolded to $\phi \equiv (a \land \ltlGlobally a) \land (\lnot a \land \ltlGlobally \lnot a) \equiv \false$.

\subsubsection{Initializing strategies based on trueness} can be achieved as follows.
Fix some game $\GraphGame$ with a (co-)safety objective and labelling function $L : \Vertices \to \LTL$.
The strategies $\strategy_0$ and $\strategy_1$ are called \emph{trueness-optimal} if they satisfy
\begin{align*}
	\strategy_0(v_0) & \in \argmax_{(v_0, u) \in \Edges} \trueness(L(u)) & \strategy_1(v_1) & \in \argmin_{(v_1, u) \in \Edges} \trueness(L(u))
\end{align*}
for all vertices $v_0 \in \VerticesSys$ and $v_1 \in \VerticesEnv$, respectively.
Observe that, since we assumed the game to be alternating, all $u$ vertices in the above equations belong to the respective opponent.

This immediately yields our first semantic algorithm $\texttt{SI}_{sem}$, which runs \texttt{SI} initialized with trueness optimal strategies.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[auto,node distance=2cm,initial text=]
		\node[systemltl,initial left] (s0) {$(a \lor \ltlNext \phi) \land \ltlNext \ltlFinally \psi$};
		\node[environmentltl] [right=1cm of s0] (s1) {$\ltlFinally \psi$};
		\node[environmentltl] [below=0.5 cm of s1] (s2) {$\phi \land \ltlFinally \psi$};
		\node[cloud, draw, cloud puffs=10,aspect=1.5] [right of=s1] (s1dots) {$\dots$};
		\node[cloud, draw, cloud puffs=10,aspect=1.5] [right of=s2] (s2dots) {$\dots$};

		\path[->]
			(s0) edge node {$a$} (s1)
			(s0) edge[swap] node {$\overline{a}$} (s2)

			(s1) edge (s1dots)
			(s1) edge (s2dots)
			(s2) edge (s1dots)
			(s2) edge (s2dots)
		;
	\end{tikzpicture}

	\caption{
		An example showing the application of trueness initialization.
		For readability, we only show the vertex labels.
		$\phi$ and $\psi$ are some non-trivial LTL formulae.
	} \label{fig:example_safety}
\end{figure}

For a small example, consider the simplified part of a game depicted in \cref{fig:example_safety}.
Here, the system player can choose whether or not to play $a$ in the initial vertex.
The successors' trueness value, namely $\trueness(\ltlFinally \psi) = \frac{1}{2}$ and $\trueness(\phi \land \ltlFinally \psi) \leq \frac{1}{4}$ (for a non-trivial $\phi$), suggest the natural choice of $a$, leading to $\ltlFinally \psi$.
Intuitively, $\ltlFinally \psi$ is \enquote{easier} to satisfy than $\phi \land \ltlFinally \psi$.
Observe that without the labelling and its trueness value this choice would not be as obvious, since the impact of this decision may only become visible much later in the game.
Quite surprisingly, this initialization solves a \emph{majority} of randomly generated games \emph{instantly} without the need for any further improvements step, as shown in the experimental evaluation.

%
%We mention that a new version of the tool \texttt{Strix} \cite{DBLP:conf/cav/MeyerSL18} uses a very similar heuristic for reachability and safety games.
%This heuristic was discovered independently and is based on a different perspective.
%Furthermore, the authors do not (yet) apply this idea in the context of general parity games. \todo{good?}


\subsection{Parity games}

To apply our ideas to parity games, there are several hurdles to overcome.
Recall that the labelling we obtain for these games has a non-trivial structure, compared to the singleton labelling in the special cases.
Hence, we cannot use the trueness value directly.
Rather, we need a more intricate way of deriving meaning from the labelling.
Because of its simplicity, we decided to use Q-learning.
Recall that Q\=/learning usually works with a single agent, interested in maximizing the obtained reward.
In our case, we instead have two antagonistic agents and we need to adapt the Q-learning framework to this setting.
Furthermore, there are some technical peculiarities when we want to incorporate priorities and the labelling.

\begin{remark}
	We again stress that our main goal is to show the usefulness of the so far unexploited semantic labelling.
	In particular, the exact approach to extracting rewards or even the fact that we use Q-learning is of secondary importance for our research goal.
	Using more advanced techniques, e.g., extract reward from the formula using neural networks, is left for future work.
\end{remark}


\subsubsection{Basic concepts}

For all variants, our Q-values lie between $-1$, corresponding to a presumably guaranteed loss for the system player, and $+1$, analogously corresponding to a win.
As usual in Q-learning, we repeatedly sample paths and update vertex values.
But, since the two players are antagonistic, we don't always pick a maximizing action while sampling.
Instead, we choose a successor with maximal Q-value in system vertices and a minimal one in environment vertices.
Once we encounter a vertex for a second time and consequently would enter a loop, we stop the sampling.

In the following we present three variants of Q-learning.
The first, agnostic variant obtains rewards only based on whether an episode is winning or losing.
This approach is widely applicable, since basically no domain knowledge is necessary.
Not surprisingly, it also is not too efficient.
We then present a first adaption, which additionally incorporates priorities.
This variant is tailored towards parity games, but does not employ any semantic information provided by the labelling.
Our experiments show that it outperforms the first variant, but only by a slim margin.
Finally, we present our semantic approach, which on top also considers the labelling, employing the trueness function in several ways.
In our experiments, this significantly outperforms the first two ideas and, on some datasets, even beats strategy improvement by a large factor.
Note that each variant also incorporates the reward signals of the previous approaches.

%Since we never visit a vertex twice during one learning episode, we can delay the reward propagation until we obtained the whole path.

\subsubsection{Rewards based on winning paths} are binary, yielding $+1$ for winning and $-1$ for losing.
In our case, this means that when we stop sampling after entering a loop, we determine whether the loop is winning or losing and propagate the value accordingly.
We initialize the Q-values with $0$, since there is no a-priori information available.
The resulting Q-learning variant is denoted by $\texttt{QL}_{win}$.

\subsubsection{Priority rewards} are the first step to a more intricate reward signal.
Here, the agent additionally obtains intermediate rewards based on the priority of the edge.
Recall that these priorities are natural numbers, and the system player is interested in large, odd priorities.
Dually, large even priorities should be avoided.

There are two difficulties associated with this idea.
Since we assumed our Q\=/values to lie between $-1$ and $+1$, we need to rescale the priorities into this domain.
Furthermore, we need to rescale them such that larger priorities significantly \enquote{overrule} smaller ones, reflecting the nature of the parity objective.
For example, obtaining ten $5$ priorities in a row is irrelevant if afterwards one $6$ is encountered.

We approach this problem by rescaling the priorities as follows.
Let $p_i$ be the priorities occurring in the given game, sorted in ascending order.
We first compute the absolute frequency of each priority as $f(p_i) = \cardinality{\{s \mid \priorityAssignment(s) = p_i\}}$, i.e. the number of vertices in the whole game labelled with priority $p_i$.
Then, we define the scaled priorities $\overline{p}_i$ by $\overline{p}_0 = p_0$, $\overline{p}_i = 2 \cdot f(p_{i-1}) \cdot \overline{p}_{i-1} + 1$.
Observe that $\overline{p}_i$ is larger than the sum of all $\overline{p}_j$ with $j < i$ occurring in the game.
Finally, we re-normalize $\overline{p}_i$ into the $[-1, +1]$ domain by $r_i := (-1)^{p_i + 1} \overline{p}_i (1 + \sum_j \overline{p}_j \cdot f(p_j))^{-1}$
Even priorities are mapped to the negative domain, as the system player wants to avoid them.
As before, we initialize the Q-values with $0$.

We denote this Q-learning variant by $\texttt{QL}_{pri}$.
Note that this approach is applicable to general parity games.
In our case, it indirectly uses the labelling, since the priorities of the game are directly derived from the labelling and correspond to progress in the monitors.
%Recall that rewards are the central driving force of Q-learning.
%Hence, we need to design a reward function which incentives winning paths of the system player.
%We introduce three different reward signals.

\subsubsection{Semantic rewards} are our idea for exploiting the information provided by the vertex labelling, denoted by $\texttt{QL}_{sem}$.
Firstly, we describe how we assign the initial Q-values.
%A good choice of initial values can significantly affect the performance of Q-learning, as mentioned earlier.
Recall that we cannot apply the trueness value to the whole labelling, since in general it comprises several different LTL formulae corresponding to different goals.
Nevertheless, we can still easily exploit the master formula to obtain a sensible value.
In particular, we initialize the Q-value of each action based on the trueness of the master formula in the successor vertex.
This directly generalizes the approach of the special case of (co-)safety, where the labelling consists only of the master formula.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
		\node[systemltl,initial left] (s0) {$\ltlGlobally \ltlFinally (a \land \ltlNext b); [a \land \ltlNext b]$};
		\node[systemltl,right=1.5cm of s0] (s1) {$\ltlGlobally \ltlFinally (a \land \ltlNext b); [b]$};

		\path[->]
			(s0) edge[out=20,in=160] (s1)
			(s0) edge[loop above] (s0)

			(s1) edge[out=200,in=-20] (s0)
			(s1) edge[loop above] (s1)
		;
	\end{tikzpicture}
	\caption{A simplified example for a monitor labelling as produced by \texttt{Rabinizer}.
	The first formula represents the master formula, while the second one corresponds to the only monitor's formula.
	} \label{fig:example_labelling}
\end{figure}

Now, we introduce our ideas for deriving the reward signal from the labelling.
Recall that apart from the master formula we have several monitor formulae, corresponding to goals which we have to fulfil repeatedly.
We present a motivating example in \cref{fig:example_labelling}.
There, we show a (simplified) labelling produced for the formula $\psi = \ltlGlobally \ltlFinally (a \land \ltlNext b)$.
In order to satisfy $\psi$, we repeatedly need to play $a$ and then in the next step $b$.
The master formula is the same in both vertices, hence we need to analyse the monitors instead.
Intuitively, playing $a$ seems to be the more natural choice in the initial vertex, since $b$ is easier to satisfy than $a \land \ltlNext b$.
Hence, our main idea is to also apply trueness analysis to the monitor labels.

%Additionally, recall that monitors are (roughly) ordered according to their importance.
%Failing a highly-ranked monitor will incur a high cost, i.e. a large, even priority.

Consequently, the system player should be interested not only in the ad-hoc reward obtained by following good priorities, but also in \enquote{progressing} other monitors.
To this end, we also give a reward proportional to the change in trueness for all monitors which are ranked higher than the current priority as follows.

Let $e = (u, v)$ be an edge in some game $\GraphGame$ with priority assignment $\priorityAssignment$ and labelling $L$.
By taking this edge, each monitor updates its monitored formulae.
In particular, some monitor may fail or succeed due to this transition.
Let $m_e$ be the index of the highest-ranked of such failing or succeeding monitors in the labelling of vertex $u$.
If there is no such monitor, let $m_e = -1$.
Then, all monitors ranked higher than $m_e$ made some progress, but did not fail or succeed.
Nevertheless, the system player is interested in succeeding at least one of those monitors and let none of them fail.
Hence, we incentivise the system player to take actions which additionally bring monitors closer to succeeding or at least do not worsen their state.
As basis for this approximation, we again use the trueness value.
Note that we still use the winning and priority based rewards, hence the \enquote{progress} of the monitor at $m_e$ is already incorporated.

Each monitor is a list of formulae which all have to be fulfilled repeatedly.
Since we want all of these goals to be satisfied, we first take the minimum trueness value for all formulae tracked by a particular monitor.
Furthermore, since the progress of all monitors ranked lower than $m_e$ is irrelevant due to the success or fail event of $m_e$, we ignore them.
Together, we are left with one value for each monitor ranked higher than $m_e$.
To aggregate these values, we pick the maximal one, letting the learner focus on improving a single monitor instead of slowly progressing all of them.
The overall \enquote{progress} reward thus is given by
\vspace{-0.25em} %
\begin{equation*}
	\mathsf{progress} = \max_{m > m_e} \left( \min_{\phi \in L(v)_m} \trueness(\phi) - \min_{\phi \in L(u)_m} \trueness(\phi) \right), \vspace{-0.25em} %
\end{equation*}
where $L(v)_m$ are the formulae tracked by monitor $m$ in vertex $v$.
%For the overall reward, we combine the priority reward and progress reward by a weighted average.

Note that this is only one of many possible choices.
Since we are only interested in showing the general applicability of our idea, we simply picked the best heuristic out of several hand-crafted definitions of $\mathsf{progress}$.
%For example, we also tried variants where some of the $\min$ aggregations are replaced by a $\max$ or (geometric) averages.
%Most of these variants performed comparable, but slightly worse than the above definition in our evaluation.

==> 4_implementation.tex <==
\section{Implementation} \label{sec:implementation}

Maybe put training section here?

